Traffic Forecasting using Vehicle-to-Vehicle Communication

We take the first step in using vehicle-to-vehicle (V2V) communication to provide real-time on-board traffic predictions. In order to best utilize real-world V2V communication data, we integrate first principle models with deep learning. Specifically, we train recurrent neural networks to improve the predictions given by first principle models. Our approach is able to predict the velocity of individual vehicles up to a minute into the future with improved accuracy over first principle-based baselines. We conduct a comprehensive study to evaluate different methods of integrating first principle models with deep learning techniques. The source code for our models is available at https://github.com/Rose-STL-Lab/V2V-traffic-forecast .

==> scraps.tex <==

% % % Version 1:  Test/Train split1 2000-7000, 7000-8000, 8000-end
% % dataset1_car1tocar3.mat
% % % %  V2V Traffic Prediction LSTM-Velocity.ipynb
% % % %  V2V_Traffic_Prediction_LSTM Velocity 30s ego.ipynb
% % % %  V2V_Traffic_Prediction_LSTM Velocity 30s.ipynb
% % % %  V2V Traffic Prediction LSTM - Official.ipynb
% \begin{table}[ht]
% \begin{center}
% \begin{tabular}{l|ccccc}
% \toprule
% Model &  AVE@10s & VE@5s & VE@10s & VE@20s & VE@30s  \\
% \midrule
% %Constant Velocity  & 0.992 m/s & 1.008 m/s & 1.973 m/s & \\  %Tamas #'s
% Constant Velocity  & 0.992 m/s & 1.008 m/s & 1.459 m/s & 1.806 m/s & 1.962 m/s \\
% %Newell (translated)   & 5.63 m/s & 5.663 m/s & 6.353 m/s &  \\ %Tamas #'s
% Newell (translated)   & 1.591 m/s & 1.549 m/s & 1.732 m/s & 2.720 m/s & 3.411 m/s\\
% \texttt{Ego-only LSTM-FC} & 1.118 m/s &  1.219 m/s & 1.622 m/s & 1.853 m/s & 3.089 m/s \\
% %VelLSTM-FC  & 1.435 m/s & 1.648 m/s & 2.111 m/s \\
% \texttt{VelLSTM-FC}  & 0.931 m/s & 0.990 m/s & 1.412 m/s & 1.644 m/s & 1.569 m/s \\
% \texttt{ResLSTM-FC} & 1.720 m/s & 1.940 m/s & 2.778 m/s & 3.816 m/s & 5.259 m/s\\
% \bottomrule
% \end{tabular}
% \caption{Forecasting accuracy at $t=5,10,20,30$ seconds.}
% \label{table:accuracy}
% \end{center}
% \end{table}


% Split2: Test/Train split 1000-2500 & 6500-8000 (train), 3500-4000 (test), 5000-5500 (validation)
% Split3: Test/Train split valid 1000-1700 & test 2700-3400 train, 4400-8000
% dataset1_car1tocar3.mat
% dataset5_car2tocar4.mat
% \begin{table}[ht]
% \begin{center}
% \begin{tabular}{l|ccccc}
% \toprule
% Method & VE@10s & VE@20s & VE@30s & VE@40s & AVE@40s   \\
% \midrule
% Constant Velocity  & $4.97$   & $4.34$  & $4.45$  &  $5.48$ &    $4.32$ \\
% Newell (translated)   &  $5.27  $ & $5.62$  &  $4.87$ & $4.05$  &  $5.24$   \\
% Ego-only LSTM-FC & $5.54 $ & $6.09$ & $6.35$ & $6.10$ & $5.55$    \\
% VelLSTM-FC  & $4.44 \pm 0.40$  & $5.01 \pm 0.68$ & $7.10 \pm 0.84$ & $6.41 \pm 0.83$ & $5.20 \pm 0.44$       \\
% ResLSTM-FC & $5.7\pm0.2$   &  $5.2 \pm 0.02$ & $5.3 \pm 0.01$  &  $5.2 \pm 0.01$ &  $4.9 \pm 0.03$    \\
% \bottomrule
% \end{tabular}
% \caption{All numbers are in m/s.  Forecasting accuracy at $t=10,20,30,40$ seconds.  Errors are shown plus or minus one standard deviation over five runs with random seeds.}
% \label{table:accuracy}
% \end{center}
% \end{table}


% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=6.5cm,trim=20 0 30 20,clip]{figures/300K_20H_50FL_LR0005_test_sample2_100_final.png}
%     \includegraphics[width=6.5cm]{figures/errorovertime.png}
%     \caption{Left: A sample from the test set prediction 100 timesteps = 10s.  The green line is the ground truth.  Our model \texttt{ResLSTM-FC}'s prediction is purple, whereas the Newell prediction is red.  In this plot the lead car's velocity is shifted in time $v_{\rm L}(\theta-T)$ as in Section \ref{sec:background}. Right: Prediction errors grows over time for all methods. Velocity error shown is the average over the test set.}
%     \label{fig:test_final}
% \end{figure}
